ZOBNN: Zero-Overhead Dependable Design of Binary Neural Networks with Deliberately Quantized Parameters

Low-precision weights and activations in deep neural networks (DNNs) outperform their full-precision counterparts in terms of hardware efficiency. When implemented with low-precision operations, specifically in the extreme case where network parameters are binarized (i.e. BNNs), the two most frequently mentioned benefits of quantization are reduced memory consumption and a faster inference process. In this paper, we introduce a third advantage of very low-precision neural networks: improved fault-tolerance attribute. We investigate the impact of memory faults on state-of-the-art binary neural networks (BNNs) through comprehensive analysis. Despite the inclusion of floating-point parameters in BNN architectures to improve accuracy, our findings reveal that BNNs are highly sensitive to deviations in these parameters caused by memory faults. In light of this crucial finding, we propose a technique to improve BNN dependability by restricting the range of float parameters through a novel deliberately uniform quantization. The introduced quantization technique results in a reduction in the proportion of floating-point parameters utilized in the BNN, without incurring any additional computational overheads during the inference stage. The extensive experimental fault simulation on the proposed BNN architecture (i.e. ZOBNN) reveal a remarkable 5X enhancement in robustness compared to conventional floating-point DNN. Notably, this improvement is achieved without incurring any computational overhead. Crucially, this enhancement comes without computational overhead. \ToolName~excels in critical edge applications characterized by limited computational resources, prioritizing both dependability and real-time performance.

==> background.tex <==
\section{BNN PRELIMINARIES}
\subsection{Deep Neural Network}
When provided an input x ∈ R
n with n-dimension, a DNN
Fθ will map to one of C classes in common classification
tasks. More precisely, the output y ∈ R
m of the DNN is
a so-called softmax—a probability vector for C classes. In
other words, the yi
is the probability that the input x belongs
to the ith class. An input x is inferred as class i if yi has
the highest probability, so that the output class label z is
argmaxi∈[1,C] yi [20].
Generally, the DNN model Fθ is trained with a number of
samples with annotated ground-truth labels—training dataset.
The trainable parameter θ is comprised of weights and biases,
which will be learned during the training phase. Specifically,
suppose that the training dataset is a set, Dtrain = {xi
, yi}
S
i=1
of S samples, where xi ∈ R
n and corresponding groundtruth labels zi ∈ [1, C]. The training is to learn parameters
that minimize the errors between inputs predictions and their
ground-truth labels, which can be evaluated by a loss function
L. Parameters Θ after training are expressed as:
Θ = argmin
Θ∗
X
S
i
L(FΘ(xi), zi). (1)
Notably, to have accurate inference, the DNN always uses
many layers. Thus, a huge number of parameters need to be
trained and stored. In the inference stage, the computation
and storage overhead are highly related to the size of the
DNN model. In addition, the parameters are expressed with
a precision of float32 by default, so the inference is
performed based on the intensive floating-point operations
(FLOPS).
\subsection{BNN}
In the literature, a number of model compression techniques
have been proposed to reduce the memory footprint and
the computation overhead. Among these techniques (such
as pruning for trimming off less important parameters [21],
knowledge distillation for transferring knowledge from a large
model to a small one [22]), and model quantization [23] is one
of the most efficient solutions. Compared with a full-precision
model that uses floating points, a quantized model compresses
the original model weights by representing the model weights
with lower precision while retaining the inference accuracy.
The ultimate quantization is binarization, which results in
the binary neural network (BNN), such approach can play a
significant role in maximizing memory utilization for resourceconstrained IoT devices.
Binarization is a 1-bit quantization, where a parameter has
only two possible values, namely -1/0 or +1. When training
a BNN model, only 1-bit is used to represent both weight w
and activation a parameters. Following [14], binary functions
are expressed as follows:
Qw(w) = αbw, Qa(a) = βba,
where bw and ba represent the binary weight and activation,
and each is multiplied by a scale factor of α or β. The sign
functions of Qw and Qa for binarization are as follows:
\subsection{DNN model}



\label{sec:proposed}
In this section, we first describe conventional BNN models used
for  implementation. We then introduce a recently proposed
BNN model that has achieved a dramatic improvement in accuracy.



 \begin{figure}[!h]
 	\begin{center}
 	    %\vspace{-0.1in}
 		\includegraphics[width = 0.5\textwidth]{figure/binary.pdf}
 		\vspace{-0.15in}
 		\caption{In binary neural network we can change add and multiply operations to xnor and pop Count which is more hardware friendly}
 		\vspace{-0.1in}
 		\label{fig:Binary_network}
 	\end{center}	
 \vspace{-0.1in}
 \end{figure}
Binary neural networks are the extreme case of quantization. These networks take advantage of a low memory footprint. Furthermore, if we binarize both feature maps and weights, then the hardware implementation can be done by xnor and pop-count operations like Figure \ref{fig:Binary_network}. Because these operations are more hardware-friendly compare to multipcation and add operations, they result into power efficiency and significant acceleration\cite{hubara2016binarized,rastegari2016xnor}.

\subsection{BNN model}
Most recently, a more accurate BNN model named ReActNet [30],
is proposed to mitigate the accuracy gap between the binarized
model and its full-precision counterpart. The building blocks of
ReActNet is shown in Figure 3

The building block used in our baseline BNN model is illustrated
in Figure 5. 


\subsection{BNN architecture.}
 Another comprehensive line of work
explores architectural changes to strive for better model
quality. Many of them aim to incur negligible compute
and parameter overhead. For example, a channelwise realvalued rescaling of the binarized tensors can effectively mitigate the quantization loss [2,7,42]. Connecting the unquantized input activations of a binarized convolutional layer to
its output with a shortcut enhances the gradient flow and the
model representation capacity [35]. Squeeze-and-excitation
(SE) [22] is another computationally cheap technique that
promises quality improvement on small convolutional models including BNNs [36]. FracBNN [50] includes additional
BatchNorm Layers [24] in a BNN to speed up convergence.
Authors in [8] first show that using a PReLU function [16]
after each convolutional layer improves binary model quality. Along this line, it is recently reported that introducing
learnable biases into the PReLU function leads to extra improvements in model accuracy [33, 34]. With the evolution,
current BNNs finally exceeded 70% top-1.

\subsection{ Network Topology Structure}

Network architectures can affect BNN performance. ABC-Net(Lin, Zhao, and Pan, 2017), CBCN(Liu et al.,
2019a), Bi-Real-Net(Liu et al., 2018), WPRN(Mishra et al., 2017), Group-Net(Zhuang et al., 2019), BBGNet(Shen et al., 2020) and Real-to-Bin(Martinez et al., 2020) propose to modified classical network(e.g
ResNet) to improve accuracy performance. BENN(Zhu, Dong, and Su, 2019) proposes to leverage ensemble
BNN to improve prediction performance. BinaryDenseNet(Bethge et al., 2019) proposes methods and constructs customized BNN special dense network to improve accuracy performance against similar model size
BNN. Search Accurate(Shen et al., 2019) and DMS(Li et al., 2020), via designing search algorithm, adjust
the number of channel to close the accuracy gap compared to full-precision network. BATS(Bulat, Martinez,
and Tzimiropoulos, 2020a) , BNAS(Kim, Singh, and Choi, 2020), NASB(Zhu, Al-Ars, and Hofstee, 2020)
and High-Capacity-Expert(Bulat, Martinez, and Tzimiropoulos, 2020b), through designed NAS methods,
search architectures for BNN to compare accuracy performance with other BNNs which have similar model
sizes and binarized from classic network(e.g. ResNet). Especially, High-Capacity-Expert(Bulat, Martinez,
and Tzimiropoulos, 2020b) first applied condition computing within BNN called expert convolution and
combined it with grouped convolution. Inspired by MobileNet-v1, MoBiNet-Mid(Phan et al., 2020b) and
Binarized MobileNet(Phan et al., 2020a) propose new BNN architecture with high accuracy performance,
fewer ops and lighter model size. MeliusNet(Bethge et al., 2020b) and ReActNet(Liu et al., 2020c) designs
new BNN architectures which can beat the accuracy rate of full-precision light-weight MobileNet with fewer
OPs computation cost. Inspired by BN-free(Brock et al., 2021), BNN-BN-free(Chen et al., 2021) replaces
the batch normalization(BatchNorm) with scaling factor and the ReActNet without BatchNorm still has
competitive classification top-1 accuracy on the ImageNet dataset. FracBNN(Zhang et al., 2021) extends
ReActNet’s topology, re-balances the blocks of networks and designs a two 1-bit activation scheme to improve
feature learning. FracBNN has a competitive top-1 prediction result on the ImageNet dataset compared to
full precision MobileNet-v2. BCNN(Redfern, Zhu, and Newquist, 2021) designs a customized structure for
ImageNet classification with lower model size compared to MeliusNet and ReActNet






==> binary.tex <==
\section{binary neural networks}\label{}

Compared with the full-precision neural network, the binary neural networks based on 1-bit representation replace the floating-point multiplication and addition operations by the efficient XNOR-Bitcount operations, and thus largely reduce the storage space and the inference time. 

\cite{liu2020reactnet}
\cite{zhang2021fracbnn}
\cite{xu2021recu}
\cite{redfern2021bcnn}
\cite{chen2021bnn}
\cite{8782505}

2.2 Binarized Neural Networks
In 2015, Courbariaux et al. proposed BinaryConnect, a
method of training DNNs where all propagations (both forward and backward step) use binary weights [3]. In 2016,
they expanded on this work with BinaryNet and formally introduced Binarized Neural Networks (BNNs) [2]. The second paper provides implementation details on how to perform efficiently binary matrix multiplication, used in both
fully connected and convolutional layers, through the use of
bit operations (xnor and popcount). In BNNs, all weights of
filters in a layer must be −1 or 1 (which is stored as 0 and 1
respectively) instead of a 32-bit floating-point value. This
representation leads to much more space efficient models
compared to standard floating-point DNNs. A key to the success of BNNs it the binary activation function, which clamps
all negatives inputs to −1 and all positive inputs to 1. XNorNet provides a different network structure for BNNs where
pooling occurs before binary activation [8]. In this paper, we
use the BNN formulation described in the BinaryNet paper.
These networks have been shown to achieve similar performance on several standard community datasets when
compared to traditional deep networks that use float precision. Research on BNNs thus far has primarily focused on
improving the classification performance of these binary network structures and reducing the training time of the networks on GPUs. While the 32x memory reduction from
floats to bits of the weights makes BNNs an obvious candidate for low-power embedded systems, current BNN implementations are for large GPUs written in one of several
popular GPU frameworks (Theano, Torch) [10, 1]. However,
the computational model of GPUs is organized for high parallelism by reusing large temporary buffers efficiently. This
computational model is a poor fit for embedded devices that
have no hardware-supported parallelism and has only a relatively small amount of memory. In Section 3, we show that
the optimal order of computation changes drastically when
transitioning from a GPU environment with large memory
and high parallelism to an embedded environment with small
memory and no parallelism. Our implementation optimizations based on computation reordering are general and can
be applied to other BNN structures.



==> study.tex <==
\section{THE IMPACT OF Fault ON BNN Rigorous Fault Assessment in NN Architecture}\label{}


\subsection{Fault tolerant Intuition}

The key intuition of our proposed defense RA-BNN is inspired by the BNN’s intrinsic improved robustness against adversarial weight noise.


\subsection{Common BNN Architectures}
In this section, we first survey the major ML functions within the state-of-art BNN models in different domains, and then discuss their ..... Most of these models are comprised of DNNs.

\begin{itemize}
    \item Image classification: LeNet [48], AlexNet [47], VGGNet [72], Inception [75–77], ResNet [36]. Some of these networks [36, 47, 72, 76] are the winning architectures that achieve the best performance on the ILSVRC challenges [24] from 2012 to 2017. 
    \item Object detection: Faster-RCNN [66], YoLo [63], DarkNet [64]. These networks produce outstanding performance in object detection (e.g., can detect over 9000 categories [64]) and we are primarily interested in the ML thread for classification as these networks include both object localization and classification. 
    \item Steering models: Nvidia DAVE system [19], Comma.ai’s steering model [5], Rambo [12], Epoch [7], Autumn [3]. These models are the popular steering models available in the open-source community and are used as the benchmarks in related studies [59, 78].
    \item Health care and others: Detection of atrial fibrillation [80]; arrythmia detection [60]; skin cancer prediction [26]; cancer report analysis [81]; aircraft collision avoidance system [44].
\end{itemize}

These tasks are important in safety-critical domains (e.g., selfdriving cars, medical diagnosis). We are interested in those computations for calculating the results (e.g., those in hidden layers). Note that errors in the input layer such as during the reading the input image are out of consideration. The computations are summarized in Table 1.

\begin{table}[!h]
\label{T:equipos}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Basic & Conv; MatMul; Add (BiasAdd) & \\
\hline
Activation & ReLu; ELu;&\\
\hline
Pooling & Max-pool; Average-pool&\\
\hline
Normalization & Batch normalization(BN);
Local Response Normalization(LRN) &\\
\hline
\end{tabular}
\end{center}
\caption{ Major computations in state-of-art DNNs}
\label{Tab:ac_md}
\end{table}


We next discuss how most of the computations used in the above tasks are monotonic.

\begin{itemize}
    \item Basic: Convolution computation (Conv) is mainly used in the kernels in DNNs to learn the features;
    \item Activation: Activation (Act) function is often used to introduce non-linearity into the network, which is important for the network to learn non-linear complicated mappings between the inputs and outputs [34]. A widely used activation function is Rectified linear unit (ReLu) [57]
    \item Pooling: Pooling is usually used for non-linear down sampling. Max-pooling and average-pooling are the two major pooling functions.
    \item Normalization: Normalization (Norm) is used to facilitate the training of the network by dampening oscillations in the distribution of activations, which helps prevent problems like gradient vanishing [41].
    \item Data transformation: There are computations that simply transform the data, e.g., reshape the matrix, and not alter the data value. Dropout is considered as an identity mapping since it performs dropout only in training phase [74].
    \item Others: SoftMax [37] is often used in the output layer to convert the logit (the raw prediction generated by the ML model), computed for each class into a probability within (0,1) and the probabilities of all classes add up to 1.
\end{itemize}

Thus we find that almost all the operations in Table 1 exhibit monotonicity. However, this is not an exhaustive list, e.g., there are other activation functions, some of which are non-monotonic (e.g., Swish [61], Sinusoid [28])

\subsection{Fault Propagation in DNNs}
Unlike traditional programs in which soft errors can corrupt the outputs by diverting the control flow [38], [47], faults that occur in DNNs are typically numerical deviations (e.g., change of the activation value in the feature map). Even the faults that modify connections between neurons can be modeled as numerical deviations. For example, a fault that causes the DNNs to break the connection between two neurons can be considered as a 0 value passed between them.

The output quality of the DNNs is determined by the numerical output. For classification tasks, the output for the correct label needs to be high, and for the incorrect labels, it needs to be low. For regression tasks, the output needs to be as close to the target variable as possible. Therefore, for a fault to corrupt the output of DNNs, it needs to inflict significantly large deviation at the output.

\subsection{Intuition behind Quantization}
Monotonicity. In prior work, we study the mathematical
properties of DNNs, and find that many of the computations
in DNNs (e.g., ReLu, SoftMax, multiply-accumulate (MAC))
exhibit the monotone property [13]: monotonically increasing:
f(xi) ≥ f(xj ), ∀xi > xj ; or monotonically decreasing:
f(xi) ≤ f(xj ), ∀xi > xj . For example, assume a fault occurs
at the Multiply application in the MAC operation and two
faults x1, x2 occur at different bits - x1 is at the high-order bit. The monotone property is satisfied as: |x1wi
| ≥ |x2wi
|,
where wi
is the weight. Therefore, the fault propagation effect
caused by x1 is larger than that by x2 and thus is more likely
to result in an SDC. This property has been found in the
common operations (e.g., Convolution, ReLu, etc.) employed
in common DNN architectures (e.g., VGGNet, ResNet) [13].
Thus, the fault propagation behavior can be approximated
as a monotone function. This monotone property implies that
for faults to cause large deviations at the output layer, they
should also cause large deviations at the place where they occur. This leads to the observation that critical faults tend to cluster around high-order bits (i.e., causing large value deviation), while faults at low-order bits tend to be masked and do not typically affect the output much. Thus, range restriction is analogous to “transferring” the faults from the high-order bits to the low-order bits (since the effect caused by fault is reduced), which can be tolerated by the model itself.

Mitigating critical faults. Typically critical faults in DNNs
corrupt the output by fault amplification, which would propagate a single fault into multiple values causing large value
deviations. Restricting the values in the DNNs reduces the
deviations caused by the faults, which in turn lowers the
chance of the fault to result in an SDC. This is because DNNs
inherently can tolerate small value deviations and generate
correct outputs regardless. Ranger leverages this property to
prevent critical faults from corrupting the outputs, while tolerating other faults. 




\subsection{Fault Model and Fault Injection Scenario}
2.7.7 . We perform comprehensive sequences o f off-nominal NN architecture assessment beyond the asserted boundaries and requirements, to delineate a ground-truth fault-skeleton map. To identify the most vulnerable parameters in the network topology and the data type used to represent the weights and activations, we examine the effect of both SEU and MBU on each criteria in the individual layers and across the stack o f layers.

B. Fault Injection Scenarios on BNN Inference Accelerator
The soft errors might strike either memory storage or combinational logic in the hardware accelerator that cause the precision of the results to fall behind the minimum allowable correctness. For instance, the classifier misprediction due to soft error in CNNs running on a hardware accelerator as illustrated in Fig. 1, results in intolerable incident in the mission-critical applications.

3) Fault Injection Distribution:
Uniform fault injection across layers: Fiji-FIN can uniformly inject SEUs/MBUs across the memory space and time.
It can access the specific memory space that is dedicated to
store parameters of the entire QNN topology, and launch either
SEUs or MBUs onto memory cells.
Targeted in-layer fault injection: The convolutional layers
in QNN topology are tailored with different tensor dimensions.
Thus, the classification accuracy is nonuniformly impacted
by the presence of faults in each layer. Besides, depending
on how early the failure appears in the sequence of neural
network layers, the fault can manifest itself as either drastic
misclassification or minor accuracy loss/gain. Plus, in order
to investigate the impact of soft errors on individual layer,
Fiji-FIN is extended to enable the user to target a particular
parameter in a given layer.
4) Number of Injected Faults and Their Effectiveness:
Vulnerability, in our context, defines the level to which a
bit under the fault injection may perturb inference accuracy.
Accuracy is, therefore, defined as the distance between the
network inferred output and the actual output. The distance
also referred to as loss, is formulated as below,
L(f(x; (wl)
L
l=1, s) (1)
where x and s are the input and target output for the trained
binarized network with L convolutional layers. The f(.) represents network inference computation, and L(.) is the computed
loss between the network output and target output


\subsection{Which fault rate will cause binary networks to malfunction?}
 \begin{figure}[!h]
 	\begin{center}
 	    \vspace{-0.1in}
 		\includegraphics[width = 0.4\textwidth]{figure/base.pdf}
 		\vspace{-0.01in}
 		\caption{Fault study of fracbnn on cifar10 dataset.}
 		\vspace{-0.1in}
 		\label{fig:Fault_Fracbnn}
 	\end{center}	
 \vspace{-0.1in}
 \end{figure}

We studied the effect of memory fault on Fracbnn, a state-of-the-art binary neural network. Our studies, Figure \ref{fig:Fault_Fracbnn}, show that the accuracy drops at the 1e-5 fault rate from 89.1\% to 78.0\%, and it becomes random at the 1e-3 fault rate.

\subsection{What are the layers that cause the network to malfunction?}

 \begin{figure}[!h]
 	\begin{center}
 	    \vspace{-0.01in}
 		\includegraphics[width = 0.4\textwidth]{figure/layer_wise.pdf}
 		\vspace{-0.01in}
 		\caption{layer wise fault study of fracbnn on cifar10 dataset. Each line shows the effect of fault on the parameters of these layers. between these layers only conv has binary values and other layers has floating-point parameters.}
 		\vspace{-0.1in}
 		\label{fig:Layer_wise}
 	\end{center}	
 \vspace{-0.1in}
 \end{figure}

To find the most vulnerable parts, we fault studied each layer of Fracbnn separately. Figure \ref{fig:Layer_wise} shows our fault study. Based on this figure, Floating point parameters are the most vulnerable parts. Batch normalization layers and rprelu layer have the most effect on the fault, and they fill 32.2\% and 11.9\% of memory space, respectively.
It is worth noticing that binarized parameters of convolution layers have shown a great amount of robustness under extreme memory fault(1e-3 faul rate).

Existing BNN models commonly use floating-point weights and activations in the input layer to avoid a large degradation in accuracy [2, 30, 31,
40, 51].



%  \begin{figure}[!h]
%  	\begin{center}
%  	    \vspace{-0.01in}
%  		\includegraphics[width = 0.5\textwidth]{figure/BNN.png}
%  		\vspace{-0.01in}
%  		\caption{BNN}
%  		\vspace{-0.1in}
%  		\label{fig:Layer_wise}
%  	\end{center}	
%  \vspace{-0.1in}
%  \end{figure}
 
%  \begin{figure}[!h]
%  	\begin{center}
%  	    \vspace{-0.01in}
%  		\includegraphics[width = 0.5\textwidth]{figure/BNN2.png}
%  		\vspace{-0.01in}
%  		\caption{BNN}
%  		\vspace{-0.1in}
%  		\label{fig:Layer_wise}
%  	\end{center}	
%  \vspace{-0.1in}
%  \end{figure}
 
%   \begin{figure}[!h]
%  	\begin{center}
%  	    \vspace{-0.01in}
%  		\includegraphics[width = 0.5\textwidth]{figure/quantization.png}
%  		\vspace{-0.01in}
%  		\caption{BNN}
%  		\vspace{-0.1in}
%  		\label{fig:Layer_wise}
%  	\end{center}	
%  \vspace{-0.1in}
%  \end{figure}
